MonoCoder: Domain-Specific Code Language Model for HPC Codes and Tasks

With easier access to powerful compute resources, there is a growing trend in AI for software development to develop large language models (LLMs) to address a variety of programming tasks. Even LLMs applied to tasks from the high-performance computing (HPC) domain are huge in size and demand expensive compute resources for training. This is partly because LLMs for HPC tasks are obtained by finetuning existing LLMs that support several natural and/or programming languages. We found this design choice confusing - why do we need LLMs trained on natural languages and programming languages unrelated to HPC for HPC-specific tasks? In this line of work, we aim to question choices made by existing LLMs by developing smaller language models (LMs) for specific domains - we call them domain-specific LMs. Specifically, we start with HPC as a domain and build an HPC-specific LM, named MonoCoder, which is orders of magnitude smaller than existing LMs but delivers better performance on non-HPC and HPC codes. Specifically, we pre-trained MonoCoder on an HPC-specific dataset (named HPCorpus) of C and C++ programs mined from GitHub. We evaluated the performance of MonoCoder against state-of-the-art multi-lingual LLMs. Results demonstrate that MonoCoder, although much smaller than existing LMs, outperforms other LLMs on normalized-perplexity tests (in relation to model size) while also delivering competing CodeBLEU scores for high-performance and parallel code generations. In other words, results suggest that MonoCoder understands HPC code better than state-of-the-art LLMs.

==> misc.tex <==
%The \tokom{} tokenization process involves generating an anonymized version of the original code by replacing variable names, numbers, and strings; parsing this anonymized code to create an Abstract Syntax Tree (AST); updating the AST to reflect anonymization changes and maintaining a change dictionary; converting the modified AST back into code while discarding extraneous details; splitting multi-part tokens like variable names for improved understanding; and attaching random numbers from a predefined range to recurring tokens to reduce reliance on specific replacements. This approach enhances a language model's comprehension of code structure and context, enabling better generalization and accurate code completions for high-performance computing, with the added benefit of being able to restore semantics using the change dictionary for user-friendly results.

% The Tokompiler tokenization process goes as follows:
% \begin{itemize}[wide, labelwidth=!, labelindent=0pt]

% \item \textit{Generate Replaced Code}: Create a version of the original code with anonymized variable names, numbers, and strings.
   
% \item \textit{AST Parsing}: Parse the anonymized code using tree-sitter or any suitable parser to generate an AST.

% \item \textit{Recreate AST Changes}: Update the AST to reflect the changes made during anonymization. Keep a dictionary of all changes done per file/function to facilitate restoring semantics back later.

% \item \textit{AST to Code-Tokenize}: Transform the updated AST back into code, eliminating any comments, new lines, and READMEs that may have been introduced during anonymization. This code-tokenized version will have a much smaller number of tokens.

% \item \textit{Token Splitting}: Split multi-part tokens (e.g., "var\_1" to ["var", "1"]) to ensure that the model comprehends variable names as a combination of type and a unique identifier.

% \item \textit{Random Number Attachment}: For recurring tokens (e.g., "var\_1" or "num\_2"), use statistics to attach random numbers from a predefined range (e.g., 1 to 1000) during each tokenization. The attached numbers are randomly chosen without any relation to the type or order of the replaced tokens or the file/function length.

% \end{itemize}

% By following this process, we can ensure that the model focuses on the code structure, context, and relevant semantics rather than learning specific local, unnecessary, or misleading semantics. Using random numbers and splitting tokens helps disentangle the importance of specific replacements from their roles as variables or arrays. This approach improves generalization and better code completions for high-performance code. Additionally, restoring semantics back to the user using the dictionary of changes at inference maintains the usability and interpretability of the model's results.


%Our work is also a first step towards improving the interpretability and explainability of code generated from LLMs, which are paramount for HPC practitioners to trust and validate the outcomes \cite{gottschlich2018three}.
%First, the enormous computational and memory requirements of LLMs pose a significant obstacle in their practical adoption for HPC languages and tasks \cite{xu2022systematic, li2023starcoder}. These models are often prohibitively large and demand substantial computational resources, making their deployment on standard HPC platforms challenging. Furthermore, adapting LLMs to specific HPC domains and ensuring their reliable generalization across diverse scientific and engineering applications demands further investigation \cite{yeticstiren2023evaluating, godoy2023evaluation, martinez2023code, guo2023longcoder, mukherjee2023stack}. Additionally, the interpretability and explainability of LLM-generated results are paramount for HPC practitioners to trust and validate the outcomes \cite{gottschlich2018three}.

%Ensuring reliable generalization of LLMs across diverse scientific and engineering HPC applications\footnote{Leveraging code LLMs for HPC tasks can speed up code development, generate optimized parallel implementations from high-level specifications, improve code readability and maintainability, facilitate cross-platform compatibility through code translation, optimize code for parallel execution and resource utilization, identify performance bottlenecks and parallelization issues, enable code search for existing optimized implementations, detect code duplication and bugs, suggest performance improvements, facilitate correct API usage, analyze code dependencies, and enforce performance-oriented coding standards for better overall HPC application performance.} demands further investigation \cite{yeticstiren2023evaluating, godoy2023evaluation, martinez2023code, guo2023longcoder, mukherjee2023stack}. 

%High-Performance Computing (HPC) has emerged as a cornerstone of modern scientific and computational endeavors, enabling tackle increasingly complex and data-intensive problems \cite{reed2022reinventing}.

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>10010520.10010553.10010562</concept_id>
%   <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010575.10010755</concept_id>
%   <concept_desc>Computer systems organization~Redundancy</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010553.10010554</concept_id>
%   <concept_desc>Computer systems organization~Robotics</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10003033.10003083.10003095</concept_id>
%   <concept_desc>Networks~Network reliability</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}

%\keywords{Language Models, Code Completion, High-Performance Computing, Fortran, Tokompiler, Polycoder, SPT-Code}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}
